Embryo as an active granular fluid: stress-coordinated cellular constriction chains

Mechanical stress plays an intricate role in gene expression in individual cells and sculpting of developing tissues. However, systematic methods of studying how mechanical stress and feedback help to harmonize cellular activities within a tissue have yet to be developed. Motivated by our observation of the cellular constriction chains (CCCs) during the initial phase of ventral furrow formation in the Drosophila melanogaster embryo, we propose an active granular fluid (AGF) model that provides valuable insights into cellular coordination in the apical constriction process. In our model, cells are treated as circular particles connected by a predefined force network, and they undergo a random constriction process in which the particle constriction probability P is a function of the stress exerted on the particle by its neighbors. We find that when P favors tensile stress, constricted particles tend to form chain-like structures. In contrast, constricted particles tend to form compact clusters when P favors compression. A remarkable similarity of constricted-particle chains and CCCs observed in vivo provides indirect evidence that tensile-stress feedback coordinates the apical constriction activity. We expect that our particle-based AGF model will be useful in analyzing mechanical feedback effects in a wide variety of morphogenesis and organogenesis phenomena.

==> loadIt <==
#! /bin/csh

#! /bin/csh
set texfile=article

latex $texfile
bibtex $texfile
latex $texfile
latex $texfile

xdvi -s 5 -geometry 1000x740-0+0 -interpreter /usr/bin/gs.exe $texfile&

emacs -geometry 80x43+0+0 -T 'embryo - texfiles' \
Sections/appendix.tex \
Sections/conclusions.tex \
Sections/results-and-discussion.tex \
Sections/system.tex \
Sections/background.tex \
Sections/introduction.tex \
Sections/abstract-and-title.tex&

sleep 3

emacs -geometry 80x42+20+20 -T 'embryo - figtex' \
Figtex-J/stress_evolution_pbcx.tex \
Figtex-J/stress_distribution_2x.tex \
Figtex-J/stress_distribution_1x.tex \
Figtex/microstructure_evolution.tex \
Figtex/t12pbcx-stressdist.tex \
Figtex/t2-betacomp_141.tex \
Figtex/t12pbcx-betacomp-r.tex \
Figtex/cellconstchains.tex \
Figtex/embryo_schematic.tex&

sleep 2

emacs -geometry 80x41+40+40 -T 'embryo - drivers' article.tex localdefs.sty&



==> styles-slant/slantsc/ChangeLog <==
2012/01/01  2.11  Harald Harders
	- Update e-mail address

2003/11/09  2.10  Harald Harders
	- State date and version explicitely in \ProvidesPackage

2003/09/17  2.00  Harald Harders
	- The booleans caused problems when using \fontshape
	  explicitely, which, for instance, is performed by
	  \normalfont. Thus, the new version does not use them
	  at all and now works with \fontshape.
	
2003/09/10  1.00  Harald Harders 
	- Entirely new package




==> styles-slant/slantsc/Makefile <==

SRCDIR=slantsc
INSTALLDIR=`kpsewhich --expand-path='$$TEXMFLOCAL'`/tex/latex/slantsc
DOCDIR=`kpsewhich --expand-path='$$TEXMFLOCAL'`/doc/latex/slantsc
VERSION=`pdflatex getversion | grep '^VERSION' | sed 's/^VERSION \\(.*\\)\\.\\(.*\\)/\\1_\\2/'`


.SUFFIXES: .sty .ins .dtx .pdf

.ins.sty:
	pdflatex $<

.dtx.pdf:
	pdflatex $<
	pdflatex $<
	makeindex -s gind.ist $(*D)/$(*F)
	makeindex -s gglo.ist -o $(*D)/$(*F).gls $(*D)/$(*F).glo
	pdflatex $<


all: slantsc slantsc.pdf


slantsc: slantsc.sty



clean:
	@-rm -f slantsc.{glo,gls,idx,ilg,ind,aux,log,toc}
	@-rm -f *~

distclean: clean
	@-rm -f slantsc.{sty,pdf,ps}

tar:	all clean
	echo Lege slantsc-$(VERSION).tar.gz an
	-rm -f slantsc-$(VERSION).tar.gz
	tar czCf .. slantsc-$(VERSION).tar.gz \
	  $(SRCDIR)/README $(SRCDIR)/Makefile \
	  $(SRCDIR)/ChangeLog \
	  $(SRCDIR)/slantsc.{dtx,ins,pdf} \
	  $(SRCDIR)/testslantsc.tex \
	  $(SRCDIR)/slantsc.xml \
	  $(SRCDIR)/getversion.tex
	rm -f getversion.log

zip:	all clean
	-rm -f slantsc-$(VERSION).zip
	mkdir -p tex/latex/slantsc
	mkdir -p doc/latex/slantsc
	mkdir -p source/latex/slantsc
	cp slantsc.sty tex/latex/slantsc/
	cp slantsc.pdf testslantsc.tex doc/latex/slantsc/
	cp ChangeLog Makefile slantsc.dtx slantsc.ins README source/latex/slantsc/
	zip -r slantsc-$(VERSION).zip tex doc source
	rm -rf tex doc source
	rm -f getversion.log


install: all
	if [ ! -d $(INSTALLDIR) ]; then mkdir -p $(INSTALLDIR); fi
	if [ ! -d $(DOCDIR) ]; then mkdir -p $(DOCDIR); fi
	install -m644 slantsc.sty $(INSTALLDIR)
	install -m644 slantsc.pdf $(DOCDIR)
	texhash


slantsc.sty: slantsc.ins slantsc.dtx



==> styles-slant/slantsc/README <==
slantsc.sty
===========

This package enables the use of small capitals in different font
shapes, e.g., slanted or bold slanted for all fonts that provide
appropriate font shapes.
The only prerequisite is that the corresponding |fd| file has to
define the font shapes |scsl| resp.\ |scit| for slanted resp.\
italic small capitals.


Copyright 2003, 2012 Harald Harders

This program can be redistributed and/or modified under the terms
of the LaTeX Project Public License Distributed from CTAN
archives in directory macros/latex/base/lppl.txt; either
version 1 of the License, or any later version.



Installation:

automatic: - run make
	   - run make install
	 or
           - run make
           - copy slantsc.sty to a place where LaTeX can find it
           - run texhash or the corresponding command of your distribution

by hand: - execute latex on slantsc.ins
         - execute latex on slantsc.dtx (2x)
         - copy slantsc.sty to a place LaTeX can find it
         - run texhash or the corresponding command of your distribution



2012-01-01
Harald Harders
harald.harders@gmx.de

